An Integrated Approach to AI-Generated Content in e-health

Artificial Intelligence-Generated Content, a subset of Generative Artificial Intelligence, holds significant potential for advancing the e-health sector by generating diverse forms of data. In this paper, we propose an end-to-end class-conditioned framework that addresses the challenge of data scarcity in health applications by generating synthetic medical images and text data, evaluating on practical applications such as retinopathy detection, skin infections and mental health assessments. Our framework integrates Diffusion and Large Language Models (LLMs) to generate data that closely match real-world patterns, which is essential for improving downstream task performance and model robustness in e-health applications. Experimental results demonstrate that the synthetic images produced by the proposed diffusion model outperform traditional GAN architectures. Similarly, in the text modality, data generated by uncensored LLM achieves significantly better alignment with real-world data than censored models in replicating the authentic tone.

==> remove.tex <==

% In the evolving landscape of machine learning research, Large Language Models (LLMs) are increasingly being recognized for their versatility beyond text processing tasks, extending into the realm of synthetic data generation. This innovative application is primarily facilitated through the adaptation of transformer-based architectures \cite{vaswani2017attention}, which excel in encoding intricate data relationships using self-attention mechanisms. These mechanisms adeptly weigh the significance of various elements within the input, albeit traditionally textual. However, the application to tabular data synthesis introduces unique challenges, particularly in converting structured tabular rows into a textual format that preserves the inherent data relationships. This translation process is crucial for maintaining the integrity and semantic coherence of the generated synthetic data. For this reason, incorporating LLMs in such a task is still unexplored. Also, recent researches have shown that modifying loss functions in GAN-based architectures are beneficial for downstream tasks \cite{ahmed2023structure}.

% Due to the aforementioned research gaps, the contributions of this research are crucial in advancing the domain of synthetic tabular data generation for of NIDS. We introduce two novel methodologies that significantly enhance the quality and efficacy of the generated synthetic datasets. Firstly, we present an evolved version of CTAB-GAN+, which integrates feature marching loss. Secondly, we pioneer the utilization of fine-tuned LLMs for synthetic tabular data generation. Leveraging efficient fine-tuning techniques, our method thrives even in resource-constrained settings. We also implement $k$-shot prompting strategies that condition the LLM to generate synthetic instances adhering to specific class labels, thereby maintaining class distribution and enabling controlled synthetic data production. To the best of our knowledge, this is the first instance where LLMs have been successfully adapted for such a task, showcasing their potential beyond traditional text-based applications. The contributions of this research can be summarized as follows:

% \begin{itemize}[leftmargin=*, noitemsep]
%     \item Development of an enhanced CTAB-GAN+ model with a novel feature marching loss for improved data generation fidelity.
%     \item Introduction of fine-tuning techniques for LLMs to generate high-quality synthetic tabular data in a resource-constrained environment.
%     \item First known application of LLMs for synthetic tabular data generation, setting a new precedent in the field.
% \end{itemize}



% In addition to the Wasserstein loss with gradient penalty (Was+GP), CTAB-GAN+ incorporates three additional loss terms for the generator to improve the quality of the synthetic data. The information loss matches the mean and standard deviation statistics between the real and synthetic data features, ensuring the generated samples have similar statistical characteristics. The downstream loss encourages the generator to produce samples that are predictive of the target variable, enforcing the semantic integrity of the synthetic data. Finally, the generator loss minimizes the cross-entropy between the generated output classes and the given conditional vector, helping the generator learn to produce the correct class distributions.





% 1. Information loss:
% $L_{\text{G}}^{\text{info}} = \|\mathbb{E}[\mathbf{f}_x]_{x \sim p_{\text{data}}(x)} - \mathbb{E}[\mathbf{f}_{G(z)}]_{z \sim p(z)}\|_2 + \|\text{SD}[\mathbf{f}_x]_{x \sim p_{\text{data}}(x)} - \text{SD}[\mathbf{f}_{G(z)}]_{z \sim p(z)}\|_2$

%    This loss matches the first and second-order statistics (mean and standard deviation) of the real and synthetic data features.

% 2. Downstream loss:
% $L_{\text{G}}^{\text{dstream}} = \mathbb{E}_{z \sim p(z)}[|l(G(z)) - C(\mathbf{f}_e(G(z)))|]$

%    This loss encourages the generator to produce samples that are predictive of the target variable, enforcing semantic integrity.

% 3. Generator loss:
% $L_{\text{G}}^{\text{generator}} = H(\mathbf{m}_i, \hat{\mathbf{m}}_i)$

%    This loss minimizes the cross-entropy between the generated output classes and the given conditional vector.

% The discriminator is trained using the standard Was+GP objective.

% The combination of these loss terms helps the generator produce synthetic data that is statistically similar to the real data and maintains the semantic relationships between variables.

% ## General Transform
% To address the limitations of one-hot encoding and Mode-Specific Normalization, CTAB-GAN+ introduces the General Transform (GT). GT encodes all variables, both continuous and categorical, into the range of [-1, 1] using a shifted and scaled min-max normalization:

% $x_t = 2 \cdot \frac{x - \min(x)}{\max(x) - \min(x)} - 1$

% This transformation makes the encoding directly compatible with the tanh activation in the generator, and avoids the dimensionality explosion caused by one-hot encoding.

% For categorical variables, GT first encodes the categories as integers before applying the min-max normalization, and then rounds the values back to integers after decoding.

% The justification for GT is that it provides a simpler and more efficient encoding scheme, especially for continuous variables with simple, single-mode Gaussian distributions, where the more complex VGM-based encoding is not necessary.

% ## Handling Long-tailed Distributions
% For continuous variables with long-tailed distributions, CTAB-GAN+ applies a logarithmic transformation prior to encoding with the VGM-based Mixed-type Encoder:

% $\tau_c = \begin{cases}
% \log(\tau) & \text{if } \ell > 0 \\
% \log(\tau - \ell + \epsilon) & \text{if } \ell \leq 0
% \end{cases}$

% where $\ell$ is the lower bound of the variable and $\epsilon$ is a small positive constant.

% This logarithmic compression helps the VGM model better capture the tail behavior of the distribution, improving the overall encoding quality.

% ## Differential Privacy
% To provide strict privacy guarantees, CTAB-GAN+ leverages Rényi Differential Privacy (RDP) during the training of the discriminator network. The key steps are:

% 1. Use Differentially Private Stochastic Gradient Descent (DP-SGD) to train the discriminator, with gradients clipped to a norm of 1.
% 2. Compute the RDP parameters (, ε) for each discriminator update step, using the subsampled RDP analysis:

% $(\epsilon + \frac{\log 1/\delta}{\alpha - 1}, \delta)$-RDP

% where $\alpha = 2B/\sigma^2$ and $B$ is the batch size.

% 3. Track the cumulative privacy budget using the RDP composition theorem.

% By only applying DP to the discriminator, CTAB-GAN+ ensures that the generator network remains unmodified, preserving the data utility of the generated samples.

% Together, these components of the CTAB-GAN+ methodology aim to generate high-quality synthetic tabular data that closely matches the statistical properties and machine learning utility of the original dataset, while providing rigorous privacy protections.
